PanoWorld: Geometry-Consistent Panoramic Video World Modeling

We present PanoWorld, a panoramic video world model that generates geometry-consistent 360$\degree$ video from a single image and a caption. Existing panoramic video methods optimize primarily for visual realism and do not explicitly constrain the underlying 3D scene state, producing outputs that appear plausible yet exhibit inconsistent depth, broken correspondences, and implausible motion across the spherical surface. We address this gap by framing panoramic video generation as a geometry- and dynamics-consistent latent state modeling problem rather than pure visual synthesis. Building on a pre-trained perspective video world model, we introduce two lightweight regularizers: a depth consistency loss against pseudo ground-truth panoramic depth, and a trajectory consistency loss that supervises the 3D world-frame positions of tracked points across time. We further apply spherical-geometry-aware adaptation to the conditioning and positional encoding. We additionally introduce PanoGeo, a unified geometry-aware panoramic video dataset with consistent depth, trajectory, and prompt annotations across diverse real and synthetic sources, used for both training and stratified evaluation. Experiments show that PanoWorld improves geometric consistency over prior panoramic generation methods while maintaining competitive visual realism, establishing that panoramic video generation must be treated as a geometric modeling problem to support the holistic spatial understanding requirements of embodied AI applications. Code is available at https://github.com/ostadabbas/PanoWorld.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and the bullet list of contributions in Sec.~\ref{sec:intro} state three claims: (i) framing panoramic video generation as a geometry- and dynamics-consistent state modeling problem with two auxiliary losses (depth and 3D track consistency); (ii) spherical-geometry-aware adaptation (ERP RoPE, panorama-shaped multi-path conditioning, SigLIP2 features); and (iii) the \dataset{} dataset with a stratified evaluation split. All three claims are quantitatively supported by Table~\ref{tab:main} and Table~\ref{tab:ablation}, and qualitatively by Fig.~\ref{fig:qualitative}, which show that \pano{} improves geometric self-consistency without sacrificing visual realism on \dataset{}'s evaluation split.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers.
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings.
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sec.~\ref{sec:discussion} contains an explicit \textbf{Limitations} paragraph: \pano{} generates fixed $93$-frame clips, longer rollouts would accumulate drift, and the monocular DAP depth pseudo-labels together with the perspective-video Cosmos prior introduce supervisory bias on equirectangular content. Compute requirements and per-stage compute budgets are stated in Appendix~\ref{sec:training}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper.
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not present theoretical results. All formulas (Eqs.~\ref{eq:depth_loss}--\ref{eq:track_loss}) are constructive definitions of the training losses, not theorems.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results.
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition.
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced.
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sec.~\ref{sec:method} fully specifies the architecture (panorama-shaped multi-path conditioning, ERP RoPE, depth head, two losses with explicit weights). Sec.~\ref{sec:exp_setup} specifies dataset splits and the input-parity protocol. Appendix~\ref{sec:training} lists every optimizer / loss hyperparameter (AdamW, lr $2{\times}10^{-5}$, $\lambda_d{=}0.3$, $\lambda_\tau{=}0.06$, $\sigma_{\max}{=}3.0$, $\alpha{=}0.5,\beta{=}0.25$) and the two-stage schedule, Appendix~\ref{sec:inference} fully specifies the two-round inference pipeline, Appendix~\ref{sec:supple_dataset} specifies the \dataset{} construction (sources, captioning, DAP/CoTracker3 annotation), and Appendix~\ref{sec:supple_eval} specifies metric definitions and the input-parity protocol. The base perspective prior (Cosmos~Predict~2.5, 2B post-trained), tokenizer (WAN~2.1 VAE), text encoder (Qwen2.5-VL-7B), depth model (DAP), tracker (CoTracker3), and semantic encoder (SigLIP2~So400m/14) are listed by exact public version in Appendix~\ref{sec:external_components}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable.
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We will release the training and evaluation pipeline (built on Cosmos~Predict~2.5), the \dataset{} curation and annotation scripts, the trained \pano{} checkpoints (Stage~1 / Stage~2 / EMA-fp32 / EMA-bf16), and the end-to-end ``perspective image $\rightarrow$ explorable 3D scene'' pipeline (Appendix~\ref{sec:supple_3d_pipeline}) under a permissive research license upon publication. For the double-blind submission we describe the full setup in Appendix~\ref{sec:training}--\ref{sec:supple_eval}; an anonymized code/data bundle is provided as supplementary material. Public dataset components (x360, 360DVD, Argus, Habitat) and pretrained components (Cosmos~Predict~2.5, WAN~2.1 VAE, Qwen2.5-VL, SigLIP2, DAP, CoTracker3) are redistributed under their original licenses, listed in Appendix~\ref{sec:external_components}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sec.~\ref{sec:exp_setup} states the data splits ($150$-clip evaluation, balanced $50/50/50$ across \dataset{} held-out / Argus testset / Habitat-Sim), the two-stage training schedule, and the metric panel. Appendix~\ref{sec:training} provides the full optimizer configuration, loss weights, augmentations, frozen modules, and stage-wise iteration counts. Appendix~\ref{sec:supple_eval} provides the full input-parity protocol that fixes input length, FoV, and trajectory budget across all baselines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Following common practice in panoramic and long-form video generation benchmarks, we report a single inference per (method, clip) pair and aggregate over the $150$-clip stratified split. Re-sampling each method on every clip with multiple random seeds is prohibitive at the resolution and clip length we operate ($512{\times}1024$, $93$ frames per inference, $9$ baselines $+$ ablations across two input regimes). The distributional metrics (FVD, FAED, FID) are themselves population-level statistics computed over $150$ predicted vs.\ $150$ GT clips, which absorbs per-clip generation noise; the per-clip metrics (CLIP-T, 3D-Smooth, Depth-$\sigma$, Tr-Life) are mean / median values over $150$ stratified clips.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Sec.~\ref{sec:exp_setup} and Appendix~\ref{sec:training} state that training runs on a single H100 80GB GPU with batch size $1$, $93$-frame clips, in two stages ($6{,}000$ iterations at $256{\times}512$ followed by $2{,}000$ iterations at $512{\times}1024$). Inference cost for the two-round pipeline is reported in Appendix~\ref{sec:inference} ($\sim$5.8s of generated video at $512{\times}1024$ per Round-2 call). Pseudo-label generation (DAP depth and CoTracker3 trajectories) is described in Appendix~\ref{sec:supple_dataset} as a one-off offline step that scales linearly per clip. Total compute budget, including failed exploratory runs that did not enter the paper, is roughly an order of magnitude larger than the reported runs, dominated by ablation training and offline annotation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute.
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper).
    \end{itemize}

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We have reviewed the NeurIPS Code of Ethics. The self-captured panoramic video corpus was acquired by the authors in publicly accessible spaces; every face is anonymized via Deface~\citep{xu2020centerface} prior to training and evaluation (see Sec.~\ref{sec:exp_setup} and Appendix~\ref{sec:supple_dataset}). Public datasets (x360, 360DVD, Argus, Habitat) are used under their original licenses, and external pretrained models are used under their public terms.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification: Appendix~\ref{sec:broader_impacts} discusses both sides. Positive: \pano{} can lower the cost of producing geometry-consistent immersive content for VR/AR education, telepresence, virtual touring, and embodied-AI simulators. Negative: like any high-quality video generative model, panoramic generation could in principle be misused for immersive disinformation or deepfake content; we discuss mitigations including face anonymization in the released dataset, terms-of-use on model release, and the inheritance of upstream Cosmos~Predict~2.5 safety filters.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}

\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{}
    \item[] Justification: All faces in the self-captured portion of \dataset{} are anonymized with Deface~\citep{xu2020centerface} before any training, evaluation, or release (Sec.~\ref{sec:exp_setup}, Appendix~\ref{sec:supple_dataset}). The released checkpoints and dataset will ship with terms of use that prohibit deepfake / impersonation use; the underlying Cosmos~Predict~2.5 perspective prior already includes upstream safety filters that we do not bypass during fine-tuning. Public ERP source corpora (x360, 360DVD, Argus) are redistributed only via the original publishers' channels.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters.
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All external assets are credited in the main paper and listed by exact public version in Appendix~\ref{sec:external_components}: Cosmos~Predict~2.5~\citep{agarwal2025cosmos} (NVIDIA OneWay Noncommercial License), WAN~2.1~VAE~\citep{wan2025wan} (Apache~2.0), Qwen2.5-VL-7B (Apache~2.0), SigLIP2~So400m/14~\citep{tschannen2025siglip} (Apache~2.0), DAP~\citep{lin2025depth} (per its public release), CoTracker3~\citep{karaev2024cotracker} (CC-BY-NC). Public ERP video corpora x360~\citep{chen2024360}, 360DVD~\citep{wang2024360dvd}, and the Argus YouTube test split~\citep{luo2025argus} are used under their original distribution terms, and Habitat-rendered scenes are produced from publicly available 3D assets under their original licenses.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: We introduce two new assets: (i) the \dataset{} dataset, fully documented in Appendix~\ref{sec:supple_dataset} (sources, capture protocol, captioning, depth and trajectory annotation, the stratified evaluation split, and the face anonymization preprocessing); (ii) the \pano{} model checkpoints, documented by the architecture description in Sec.~\ref{sec:method}, the two-stage training recipe in Appendix~\ref{sec:training}, and the two-round inference pipeline in Appendix~\ref{sec:inference}. Both assets will be released alongside the paper with a structured datasheet / model card and an explicit license; the anonymized supplementary bundle contains a data dictionary describing every column of the per-clip annotation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc.
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}
    \item[] Justification: We do not run crowdsourcing experiments or human-subject studies. The self-captured panoramic videos are recorded by the authors themselves in publicly accessible spaces; no third-party participants are involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper.
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector.
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerYes{}
    \item[] Justification: The study received an institutional IRB exemption based on its scope (no formal human-subject experimentation; only incidental capture of bystanders in publicly accessible spaces). As an additional safeguard, every face in the self-captured corpus is anonymized with Deface~\citep{xu2020centerface} prior to use in training, evaluation, and any release; this is documented in Sec.~\ref{sec:exp_setup} and Appendix~\ref{sec:supple_dataset}. The institution name is withheld during the double-blind review.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution.
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerYes{}
    \item[] Justification: LLMs / VLMs appear at two non-core points in our pipeline, both fully disclosed. (i) Captions for \dataset{} are produced by Gemini and cross-checked by an OpenAI model under a fixed panoramic-aware prompt template (Sec.~\ref{sec:exp_setup}, Appendix~\ref{sec:supple_dataset}); these captions are pseudo-labels consumed as training/evaluation inputs and are not part of the core method. (ii) The text-conditioning pathway of the diffusion backbone reuses Qwen2.5-VL-7B as the text encoder, which is a frozen pre-existing component of Cosmos~Predict~2.5 (Appendix~\ref{sec:external_components}); we do not modify or fine-tune it. The novel components of \pano{} (panorama-shaped multi-path conditioning, ERP RoPE, depth and 3D track losses) do not involve LLMs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

